Transfer matrix analysis of one-dimensional majority cellular automata with thermal noise

Thermal noise in a cellular automaton refers to a random perturbation to its function which eventually leads this automaton to an equilibrium state controlled by a temperature parameter. We study the 1-dimensional majority-3 cellular automaton under this model of noise. Without noise, each cell in this automaton decides its next state by majority voting among itself and its left and right neighbour cells. Transfer matrix analysis shows that the automaton always reaches a state in which every cell is in one of its two states with probability 1/2 and thus cannot remember even one bit of information. Numerical experiments, however, support the possibility of reliable computation for a long but finite time.

==> Commands.tex <==
% general mathematical abbreviations


\newcommand{\wv}{{\bf w}}
\newcommand{\sigmav}{\mbox{\boldmath$\sigma$}}
\newcommand{\Omegav}{\mbox{\boldmath$\Omega$}}
\newcommand{\hv}{\mbox{\boldmath$h$}}
\newcommand{\Hv}{\mbox{\boldmath$H$}}
\newcommand{\xv}{\mbox{\boldmath$x$}}
\newcommand{\thetav}{\mbox{\boldmath$\theta$}}
\newcommand{\Iv}{\mbox{\boldmath$I$}}


\newcommand{\is}{{\!=\!}}
\newcommand{\pprime}{{\prime\prime}}
\newcommand{\double}{{\prime\prime}}
\newcommand{\bra}{\langle}
\newcommand{\ket}{\rangle}
\newcommand{\bigbra}{\left\langle}
\newcommand{\bigket}{\right\rangle}
\newcommand{\order}{{\mathcal O}}
\newcommand{\smallo}{{\mathcal o}}
\newcommand{\sgn}{\textrm{sgn}}
\newcommand{\erf}{\textrm{erf}}
%\newcommand{\Tr}{\textrm{Tr}}
\newcommand{\id}{{\rm 1\!\!I}}
\newcommand{\one}{{\rm 1\!\!I}}
\newcommand{\openone}{{\rm 1\!\!I}}
\newcommand{\plus}{{\!+\!}}
\newcommand{\minus}{{\!-\!}}
\newcommand{\bnull}{{\mbox{\boldmath $0$}}}
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\bd}{\begin{displaymath}}
\newcommand{\ed}{\end{displaymath}}
\newcommand{\vsp}{\vspace*{3mm}}
\newcommand{\room}{\rule[-0.1cm]{0cm}{0.6cm}}
\newcommand{\bigroom}{\rule[-0.4cm]{0cm}{1.0cm}}
\newcommand{\verybigroom}{\rule[-0.7cm]{0cm}{1.3cm}}
\newcommand{\extr}{{\rm extr}}

\newcommand{\F}{{\mathcal F}}
%\newcommand{\R}{{\rm I\!R}}
\newcommand{\Zset}{{\rm I\!Z}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\real}{{\rm I\!R}}
\newcommand{\N}{{\rm I\!N}}
\newcommand{\B}{{\mathcal B}}
\newcommand{\D}{{\mathcal D}}
\newcommand{\cP}{{\mathcal P}}
\newcommand{\Z}{{\mathcal Z}}
\newcommand{\W}{{\mathcal W}}


% bold characters and symbols

\newcommand{\ba}{\ensuremath{\mathbf{a}}}
\newcommand{\bb}{\ensuremath{\mathbf{b}}}
\newcommand{\bc}{\ensuremath{\mathbf{c}}}
\newcommand{\bh}{\ensuremath{\mathbf{h}}}
\newcommand{\bk}{\ensuremath{\mathbf{k}}}
\newcommand{\bm}{\ensuremath{\mathbf{m}}}
\newcommand{\bq}{\ensuremath{\mathbf{q}}}
%\newcommand{\bs}{\ensuremath{\mathbf{s}}}
\newcommand{\bu}{\ensuremath{\mathbf{u}}}
\newcommand{\bv}{\ensuremath{\mathbf{v}}}
\newcommand{\bw}{\ensuremath{\mathbf{w}}}
\newcommand{\bx}{\ensuremath{\mathbf{x}}}
\newcommand{\by}{\ensuremath{\mathbf{y}}}
\newcommand{\bz}{\ensuremath{\mathbf{z}}}

\newcommand{\bA}{\ensuremath{\mathbf{A}}}
\newcommand{\bB}{\ensuremath{\mathbf{B}}}
\newcommand{\bC}{\ensuremath{\mathbf{C}}}
\newcommand{\bD}{\ensuremath{\mathbf{D}}}
\newcommand{\bE}{\ensuremath{\mathbf{E}}}
\newcommand{\bF}{\ensuremath{\mathbf{F}}}
\newcommand{\bG}{\ensuremath{\mathbf{G}}}
\newcommand{\bH}{\ensuremath{\mathbf{H}}}
\newcommand{\bI}{\ensuremath{\mathbf{I}}}
\newcommand{\bJ}{\ensuremath{\mathbf{J}}}
\newcommand{\bK}{\ensuremath{\mathbf{K}}}
\newcommand{\bL}{\ensuremath{\mathbf{L}}}
\newcommand{\bM}{\ensuremath{\mathbf{M}}}
\newcommand{\bN}{\ensuremath{\mathbf{N}}}
\newcommand{\bO}{\ensuremath{\mathbf{O}}}
\newcommand{\bP}{\ensuremath{\mathbf{P}}}
\newcommand{\bQ}{\ensuremath{\mathbf{Q}}}
\newcommand{\bR}{\ensuremath{\mathbf{R}}}
\newcommand{\bS}{\ensuremath{\mathbf{S}}}
\newcommand{\bT}{\ensuremath{\mathbf{T}}}
\newcommand{\bU}{\ensuremath{\mathbf{U}}}
\newcommand{\bV}{\ensuremath{\mathbf{V}}}
\newcommand{\bW}{\ensuremath{\mathbf{W}}}
\newcommand{\bX}{\ensuremath{\mathbf{X}}}
\newcommand{\bY}{\ensuremath{\mathbf{Y}}}
\newcommand{\bZ}{\ensuremath{\mathbf{Z}}}

\newcommand{\blambda}{{\mbox{\boldmath $\lambda$}}}
\newcommand{\bxi}{{\mbox{\boldmath $\xi$}}}
\newcommand{\bpsi}{{\mbox{\boldmath $\psi$}}}
\newcommand{\bphi}{{\mbox{\boldmath $\phi$}}}
\newcommand{\bomega}{{\mbox{\boldmath $\omega$}}}
\newcommand{\bsigma}{{\mbox{\boldmath $\sigma$}}}
\newcommand{\btheta}{{\mbox{\boldmath $\theta$}}}
\newcommand{\bEta}{{\mbox{\boldmath $\eta$}}}
\newcommand{\bLambda}{{\mbox{\boldmath $\Lambda$}}}
\newcommand{\bOmega}{{\mbox{\boldmath $\Omega$}}}

% hat characters and symbols

\newcommand{\hh}{\hat{h}}
\newcommand{\hk}{\hat{k}}
\newcommand{\hq}{\hat{q}}
\newcommand{\hm}{\hat{m}}
\newcommand{\hw}{\hat{w}}
\newcommand{\hx}{\hat{x}}
\newcommand{\hy}{\hat{y}}

\newcommand{\hA}{\hat{A}}
\newcommand{\hC}{\hat{C}}
\newcommand{\hG}{\hat{G}}
\newcommand{\hK}{\hat{K}}
\newcommand{\hL}{\hat{L}}
\newcommand{\hQ}{\hat{Q}}

\newcommand{\hOmega}{\hat{\mbox{$\Omega$}}}

% bold and hat characters

\newcommand{\hbh}{\widehat{\mathbf{h}}}
\newcommand{\hbk}{\widehat{\mathbf{k}}}
\newcommand{\hbm}{\widehat{\mathbf{m}}}
\newcommand{\bhw}{\widehat{\mathbf{w}}}
\newcommand{\hbw}{\widehat{\mathbf{w}}}
\newcommand{\bhx}{\widehat{\mathbf{x}}}
\newcommand{\hbx}{\widehat{\mathbf{x}}}
\newcommand{\bhq}{\widehat{\mathbf{q}}}
\newcommand{\hbq}{\widehat{\mathbf{q}}}

\newcommand{\hbK}{\widehat{\mathbf{K}}}
\newcommand{\hbQ}{\widehat{\mathbf{Q}}}

% picture drawing

\newcommand{\wcirc}{\circle{30}}
\newcommand{\bcirc}{\circle*{31}}
\newcommand{\Size}{270}
\newcommand{\BSize}{200}
\newcommand{\here}{\makebox(0,0)}
\newcommand{\wbox}{{\circ}}
\newcommand{\bbox}{{\bullet}}
\newcommand{\whitesquare}{{\framebox(1.2,1.2){}}~}
\newcommand{\whitecircle}{{\large $\circ$}}
%\newcommand{\blacksquare}{\rule{1.3\unitlength}{1.3\unitlength}~}
\newcommand{\blackcircle}{{\large $\bullet$}}


% MG specific abbreviations

\newcommand{\rate}{\tilde{\eta}}
\newcommand{\s}{\sigma}
\newcommand{\si}{\sigma}
\newcommand{\del}{{\delta_{\!N}}}
\newcommand{\hbe}{\hat{\bf e}}
\newcommand{\notdelta}{\overline{\delta}}
\newcommand{\chiR}{\chi_{\!\!\!~_R}}
\newcommand{\freq}{f}

\newcommand{\TBF}{{\vspace*{3mm}\hrule\vspace*{1mm}
\begin{center}{TO BE FINISHED}\end{center}
\vspace*{1mm}\hrule\vspace*{3mm}}}

